Towards Scalable Multi-View Reconstruction of Geometry and Materials

In this paper, we propose a novel method for joint recovery of camera pose, object geometry and spatially-varying Bidirectional Reflectance Distribution Function (svBRDF) of 3D scenes that exceed object-scale and hence cannot be captured with stationary light stages. The input are high-resolution RGB-D images captured by a mobile, hand-held capture system with point lights for active illumination. Compared to previous works that jointly estimate geometry and materials from a hand-held scanner, we formulate this problem using a single objective function that can be minimized using off-the-shelf gradient-based solvers. To facilitate scalability to large numbers of observation views and optimization variables, we introduce a distributed optimization algorithm that reconstructs 2.5D keyframe-based representations of the scene. A novel multi-view consistency regularizer effectively synchronizes neighboring keyframes such that the local optimization results allow for seamless integration into a globally consistent 3D model. We provide a study on the importance of each component in our formulation and show that our method compares favorably to baselines. We further demonstrate that our method accurately reconstructs various objects and materials and allows for expansion to spatially larger scenes. We believe that this work represents a significant step towards making geometry and material estimation from hand-held scanners scalable.

==> optimization.tex <==
\boldparagraph{Optimization at Scale} 
When it comes to large computational problems, distributed computing is key. 	
Distributed optimization methods can be categorized into centralized or decentralized algorithms, \cite{Assran2020Arxiv}.
Centralized methods have one master copy of the optimization variables which is updated by all processes. 
That's problematic when it comes to parallelization and multiple processes reading/writing simultaneously.
For decentralized methods, each processor has a local copy of the optimization variables and all those copies may differ.
That requires synchronization between processes, which and how frequently messages need to pass depends on the topology and communication complexity of the problem.
Generally, that induces a communication overhead.

We distribute the computation on a set of keyframe optimizations.
Centralized optimization variables can lead to aggregation of errors across keyframes of very different regions. 
Instead, we implement a decentralized optimization strategy that facilitates accurate local reconstructions with a soft regularizer to ensure consistency across neighboring keyframes.
To reduce the communication overhead, we employ a similar strategy as \cite{Wang2020ICLR} and let each keyframe or worker independently perform a set of base optimization steps in between computing any messages.
That approach also enables parallel processing of the set of keyframes.\\ 

How to distribute the optimization? 
Following \cite{Assran2020Arxiv}, a 'large scene' can mean many input views, large input views or many optimization variables.
A typical solution is subsampling - of either the data (batched gradient descent) or the optimization variables (coordinate gradient descent).
Thereby, the subsampling can be randomly or based on knowledge of the data/variables.

For large 3D reconstruction problems, we face large numbers of captured input data as well as a number of optimization variables that scales linearly with the scene size and cubically with the resolution.
But usually, we can exploit knowledge of both the data and the optimization variables.
In the context of room-level geometry reconstruction, the data is usually \textit{spatially split} by grouping into patches \cite{Henry2013THREEDV,Pollefeys2008IJCV,Choi2015CVPR} based on image regions.
For object-level reconstructions of geometry and materials, many reconstruction methods, \eg  \cite{Nam2018SIGGRAPH,Georgoulis2014THREEDV,Li2021CVPR}, subsample the optimization variables by type or property and iterate over the properties to optimize (geometry, normals, material maps, poses) using coordinate gradient descent - we call it a \textit{split by property}.

In contrast to those methods for geometry and material estimation, we exploit natural independence for spatially separated regions (either by distance or for front and back sides) and subsample both data and optimization variables based on a \textit{spatial split}: 
To separate regions that are not visible in the same measurements, we denote a well-spread subset of all input views as keyframes.
For each keyframe, the set of observed pixels naturally induces the optimization variables and we can then optimize over this local data and variable split using coordinate gradient descent (as the before mentioned methods do as well).
